Optimizing Multiple Multi-Way Stream Joins

We address the joint optimization of multiple stream joins in a scale-out architecture by tailoring prior work on multi-way stream joins to predicate-driven data partitioning schemes. We present an integer linear programming (ILP) formulation for selecting the partitioning and tuple routing with minimal probe load and describe how routing and operator placement can be rewired dynamically at changing data characteristics and arrival or expiration of queries. The presented algorithms and optimization schemes are implemented in CLASH, a data stream processor developed in our group that translates queries to deployable Apache Storm topologies after optimization. The experiments conducted over real-world data exhibit the potential of multi-query optimization of multi-way stream joins and the effectiveness and feasibility of the ILP optimization problem.

==> sections/__latexindent_temp.tex <==
%!TEX root = ../main.tex

\section{Introduction}\label{sec:introduction}

Processing data streams is a ubiquitous problem in data management, especially
in the context of handing large-volume streams in scale-out systems. Prominent engines like
Spark Streaming~\cite{website:spark}, Flink~\cite{DBLP:journals/debu/CarboneKEMHT15,website:flink}, Apache Storm's Trident~\cite{website:storm}, or Kafka~\cite{DBLP:journals/pvldb/WangKSPZNRKS15,website:kafka}
allow users or higher-level applications to express queries in SQL-style languages, deployed and
executed over potentially very many compute tasks in a data center. In most cases, such queries
do not merely filter or aggregate tuples from a single relation but involve {\it joins} that connect information pieces from various sources.
For instance, search-engine queries and ad-clicks need to be joined for billing purposes~\cite{DBLP:conf/sigmod/AnanthanarayananBDGJQRRSV13}
and in complex event processing, events are commonly expressed by multiple criteria that do not originate from a single sensor~\cite{DBLP:journals/pvldb/KolchinskyS18}.
Once such queries are posted, they remain registered in the system and continuously report results.
Computational resources can be shared for answering multiple queries.
Trying to share work between data stream queries is not a new idea~\cite{DBLP:conf/vldb/HammadFAE03,DBLP:conf/dasfaa/YangZWX19,DBLP:conf/sigmod/KarimovRM19},
and traditionally, sharing is done on a per-operator basis.
This means, a query execution plan is produced for each query and joins or other operators share their result with downstream operators to contribute to answer multiple queries at once.


In this paper, we propose a fine-grained and easy to rewire tuple routing scheme that enables sharing of partial results between multiple multi-way join queries.
Our approach is implemented in \sysname\footnote{https://www.youtube.com/watch?v=oZxNIwvEQDw}~\cite{DBLP:conf/sigmod/DossingerMR19}, a system for optimizing continuous queries, built on top of Apache Storm~\cite{DBLP:conf/sigmod/ToshniwalTSRPKJGFDBMR14,website:storm}.
However, the concepts are applicable to all modern streaming systems that give control over the routing between workers and access to local state.

\begin{figure}[tb]
  \centering
  \begin{tikzpicture}[xscale=1.3]
    % time line

    \draw[->] (0,0) to (5,0);

    \foreach \x in {0,0.2,...,4.8} {
        \draw (\x,0.05) -- (\x,-0.05);
      }

    \node[] at (0,-0.2){\scriptsize 0};
    \node[] at (1,-0.2){\scriptsize 10};
    \node[] at (2,-0.2){\scriptsize 20};
    \node[] at (3,-0.2){\scriptsize 30};
    \node[] at (4,-0.2){\scriptsize 40};
    \node[] at (5,-0.3){\it \scriptsize time};

    % relations

    \node[] at (-.5,0.5){$S_1$};
    \node[] at (-.5,1.0){$S_2$};
    \node[] at (-.5,1.5){$S_3$};
    \node[] at (-.5,2.0){$S_4$};

    \draw[-, dotted] (0,0.5) to (5,0.5);
    \draw[-, dotted] (0,1.0) to (5,1.0);
    \draw[-, dotted] (0,1.5) to (5,1.5);
    \draw[-, dotted] (0,2.0) to (5,2.0);

    % join result
    \fill[color = red] (1.6,1.0) circle (0.1);
    \fill[color = red] (1.2,1.5) circle (0.1);
    \fill[color = red] (1,0.5) circle (0.1);
    \draw[-, color=red] (1.6,1.0) to (1,0.5) to (1.2,1.5);


    \fill[color = green] (2.6,1.0) circle (0.1);
    \fill[color = green] (2.4,1.5) circle (0.1);
    \fill[color = lightblue] (2.2,.5) circle (0.1);
    \fill[color = purple] (1.9,2.0) circle (0.1);
    \draw[-, color=green] (2.6,1.0) to (2.4,1.5);
    \draw[-, color=lightblue] (2.4,1.5) to (2.2,.5);
    \draw[-, color=purple] (2.4,1.5) to (1.9,2.0);


    \fill[color = yellow] (4.2,1.5) circle (0.1);
    \fill[color = yellow] (4.0,2.0) circle (0.1);
    \fill[color = yellow] (3.7,0.5) circle (0.1);
    \draw[-, color=yellow] (4.2,1.5) to (4.0,2.0) to (3.7,0.5);


    \fill[color = orange] (4.8,1.5) circle (0.1);
    \fill[color = orange] (4.6,0.5) circle (0.1);
    \fill[color = orange] (4.4,2.0) circle (0.1);
    \draw[-, color=orange] (4.8,1.5) to (4.6,0.5) to (4.4,2.0);

    \foreach \x in {1,2.2,3.5,3.7,4.6} { \fill (\x,0.5) circle (0.05); } % R1
    \foreach \x in {.7,.9,1.6,2.6,3.8} { \fill (\x,1.0) circle (0.05); } % R2
    \foreach \x in {.6,1.2,1.8,2.4,3.0,3.6,4.2,4.8} { \fill (\x,1.5) circle (0.05); } % R3
    \foreach \x in {1.3,1.4,1.9,3.4,4.0,4.4} { \fill (\x,2.0) circle (0.05); } % R4

    % points in time

    \draw[blue,dashed] (1.6,-2) to (1.6,2.1); \node[] at (1.6,-2.3){$\tau_1$};
    \draw[blue,dashed] (2.6,-2) to (2.6,2.1); \node[] at (2.6,-2.3){$\tau_2$};
    \draw[blue,dashed] (4.5,-2) to (4.5,2.1); \node[] at (4.5,-2.3){$\tau_3$};

    % queries

    \draw[rounded corners, fill=white] (1.2,-1.1) rectangle node {\scriptsize $q_1 (S_1, S_2, S_3)$} (3.5,-1.6);
    \draw[rounded corners, fill=white] (1.8,-.5) rectangle node {\scriptsize $q_2 (S_2, S_3, S_4)$} (3.2,-1);
    \draw[rounded corners, fill=white] (3.4,-.5) rectangle node {\scriptsize $q_3 (S_1, S_3, S_4)$} (5,-1);


  \end{tikzpicture}
  \caption{Four streaming relations with queries that are enabled and expire over time.}\label{fig:introexample}
\end{figure}


\subsection{Problem Statement}

% What is a query?
In this paper, we consider optimizing multiple equi-join queries over streamed input relations $S_1, \dots, S_m$.
We write $S_i.a$ for naming an attribute, and $s_i.a$ for the value of attribute $a$ in tuple $s_i$. Tuples have a special attribute $\tau$ which is their timestamp.
The individual join predicates comprise predicates over pairs of relations, like $S_i.a = S_j.b$, where $a$ and $b$ are attributes of $S_i$ and $S_j$, respectively.
For each relation, a window defines the maximal time difference between a tuple of this relation and another tuple for being considered joinable.
When a tuple $s_i \in S_i$ is observed, immediately, join result tuples $s_1 \circ \dots \circ s_i \circ \dots \circ s_m$ are produced for all joinable tuples $s_1, \dots, s_{i-1}, s_{i+1}, \dots, s_m$ that arrived within the window depending on the arrival time of $s_i$.
For example, the tuples arriving at times 10, 12, and 16, marked in red in Figure~\ref{fig:introexample}, satisfy the join predicates and windows of query $q_1$.
Then the join result of this tuple is produced at time $\tau_1 = 16$, as soon as the tuple of $S_2$ arrives.

% Multi query optimization of these join queries
Given streamed relations $S_1, \dots, S_m$ and queries $q_1, \dots, q_k$ where each $q_i$ is a join query over a subset of the relations.
Then the goal is, to produce both, a selection of state to materialize on workers in a distributed environment, and a routing and probing strategy between these workers which produces the correct join result, has a low memory footprint and provides high throughput.
In order to enable efficient local join computation, cross products are avoided.
The processing scheme should adapt to changes in data characteristics and the addition of new or removal of old queries.

For example, in Figure~\ref{fig:introexample} at time $\tau_1$ query $q_1$ is known to the system, so a processing strategy optimal for this query is deployed.
This involves sending arriving tuples from $S_2$ to $S_1$ for producing an intermediate result and then sending this to $S_3$ for the complete result.
At time $\tau_2$ query $q_2$ is also incorporated into the system.
Now, tuples arriving from $S_2$ are routed differently: first to $S_3$ (marked green) in order to produce the partial join result, and then both to $S_4$ (marked purple) and to $S_1$ (marked blue) in order to produce both results for $q_2$ and $q_1$, respectively.
Both queries expire eventually and $q_3$ is installed initially with the probe strategy from $S_3$ to $S_4$ then to $S_1$.
At $\tau_3$ that data characteristics have changed and thus it is more efficient to sent $S_3$ tuples first to $S_1$ and then to $S_4$.

\subsection{Contribution and Outline}

In this paper, we make the following contributions:
\begin{enumerate}[label=\arabic*.]
  \item We provide a sound and feasible working solution for optimizing multiple multi-join queries in modern scale-out data stream processors.
  \item To do so, we provide an ILP formulation of data partitioning and probing optimization.
  \item We describe how on-the-fly rewiring of tuple routing can be realized to enable fast adaptation of shared plans and intra-plan tuple routing,
        for changing data characteristics as well as for arriving or expiring queries.
  \item We report on detailed finding of a thorough experimental evaluation and provide lessons learned in optimizing multiple multi-way join queries.
\end{enumerate}

The remainder of this paper is structured as follows. Section~\ref{sec:related_work} discusses related work
and Section~\ref{sec:preliminaries} briefly introduces fundamentals of stream join processing in scale-out environments.
Section~\ref{sec:distributing_stream_joins} describes the architectural setup and the core concepts of mating partitioning schemes imposed by equi-join predicates on tuple routing and storage.
Section~\ref{sec:join_optimization} presents the modeling of the optimization problem as integer linear program (ILP).
Section~\ref{sec:adaptive_probe_ordering} describes how tuple routing and result sharing can be adapted
to changing query load and data characteristics.
Section~\ref{sec:experiments} reports on the results of our experimental study and lessons learned.
Finally, Section~\ref{sec:conclusion} concludes the paper.

